DS3: A System-Level Domain-Specific System-on-Chip Simulation Framework

Heterogeneous systems-on-chip (SoCs) are highly favorable computing platforms due to their superior performance and energy efficiency potential compared to homogeneous architectures. They can be further tailored to a specific domain of applications by incorporating processing elements (PEs) that accelerate frequently used kernels in these applications. However, this potential is contingent upon optimizing the SoC for the target domain and utilizing its resources effectively at runtime. To this end, system-level design - including scheduling, power-thermal management algorithms and design space exploration studies - plays a crucial role. This paper presents a system-level domain-specific SoC simulation (DS3) framework to address this need. DS3 enables both design space exploration and dynamic resource management for power-performance optimization of domain applications. We showcase DS3 using six real-world applications from wireless communications and radar processing domain. DS3, as well as the reference applications, is shared as open-source software to stimulate research in this area.

==> files/extra.tex <==
% for abstract
The early evaluation of design decisions at system-level abstraction layer helps to find promising regions for subsequent development steps in lower abstraction levels by diminishing the complexity of the search problem.
%% Same idea with different words
In order to cope with the ever-increasing complexity of embedded systems, system-level descriptions are utilized to diminish the complexity of finding potentially good solutions which can then be used as initial starting points for further optimization  in lower abstraction levels.

No existing analysis tool is fit to cope with all the challenges of modern embedded system design, implying that more than one tool must be used.

architecture-independent application development/specification


To even further improve the potentials for reuse of IP
and to allow for effective exploration of alternative design
solutions, it is also widely recognized that “separation of
concerns” [3] is a crucial component in system-level design.
Two common types of separation in the design process are:
1) separating computation from communication by connecting
IP processing cores via a standard network interface
and 2) separating application (what is the system supposed
to do) from architecture (how it does it).

[3] K. Keutzer, S. Malik, A. Newton, J. Rabaey, and A. Sangiovanni-
Vincentelli, “System Level Design: Orthogonalization of Concerns
and Platform-Based Design,” IEEE Trans. Computer-Aided Design of
Integrated Circuits and Systems, vol. 19, no. 12, pp. 1523-1543, Dec.
2000.
